Advances in Constraining Intrinsic Alignment Models with Hydrodynamic Simulations

We use galaxies from the IllustrisTNG, MassiveBlack-II and Illustris hydrodynamic simulations to investigate the behaviour of large scale galaxy intrinsic alignments. Our analysis spans four redshift slices over the approximate range of contemporary lensing surveys $z=0-1$. We construct comparable weighted samples from the three simulations, which we then analyse using an alignment model that includes both linear and quadratic alignment contributions. Our data vector includes galaxy-galaxy, galaxy-shape and shape-shape projected correlations, with the joint covariance matrix estimated analytically. In all of the simulations, we report non-zero IAs at the level of several $\sigma$. For a fixed lower mass threshold, we find a relatively strong redshift dependence in all three simulations, with the linear IA amplitude increasing by a factor of $\sim 2$ between redshifts $z=0$ and $z=1$. We report no significant evidence for non-zero values of the tidal torquing amplitude, $A_2$, in TNG, above statistical uncertainties, although MassiveBlack-II favours a moderately negative $A_2\sim-2$. Examining the properties of the TATT model as a function of colour, luminosity and galaxy type (satellite or central), our findings are consistent with the most recent measurements on real data. We also outline a novel method for constraining the TATT model parameters directly from the pixelised tidal field, alongside a proof of concept exercise using TNG. This technique is shown to be promising, although the comparison with previous results obtained via other methods is non-trivial.

==> covariance.tex <==

\subsubsection{Analytic Covariance Matrix}


\begin{figure}
\includegraphics[width=1.1\columnwidth]{figures/corrmat_z0_wigner.pdf}
\caption{The correlation matrix for our fiducial \fidsim~two-point
measurements, as estimated using jackknife resampling 
(upper left triangle), and an analytic Gaussian approximation
(lower right).
Note that the two covariance matrices are symmetric about the
diagonal; the triangle configuration is shown here for illustrative
purposes only.
}\label{fig:data:correlation_matrix}
\end{figure}


In order to derive robust inferences from our measurements, 
we need a reasonable estimate for the 
covariance matrix of the data.
The full data consists of three two-point measurements for each of four snapshots;
this gives us $N = 4 \times 3 \times N_{rp}$ datapoints for each simulated
galaxy sample (96, 144 and 192 in the case of \illustris, \mbii, and \tng~respectively).
Our fiducial covariance estimate is calculated analytically. We differ in
this respect from many previous studies using hydrodynamic simulations,
which have opted to use an internal estimator such as jackknife or bootstrap
resampling.
The analytic approach carries a number of advantages, not least the ability to
extend to large scales where jackknife estimates break down.
The correlation matrix that corresponds to the 
covariance matrix calculated using the analytic method described below is
shown in the lower right triangle of Figure~\ref{fig:data:correlation_matrix}. 

Although in principle the covariance has higher order terms resulting 
from mode mixing, given the limited statistical power of the simulations
and the dominance of shot/shape noise in our measurements,
we consider the Gaussian contribution to be sufficient
for our purposes. In this paradigm, a given element is the sum of a shape (or shot) noise term
and a cosmic variance contribution:

\begin{equation}
\mathrm{Cov}\left[ w^{z_{\rm s}}_{\alpha \beta}(r_{\mathrm{p},j}), w^{z_{\rm s}}_{\delta \gamma}(r_{\mathrm{p},k}) \right ] = 
\mathrm{C}^{\mathrm{SN},z_{\rm s}z_{\rm s},kj}_{\alpha\beta\delta\gamma} +
\mathrm{C}^{\mathrm{CV},z_{\rm s}z_{\rm s},kj}_{\alpha\beta\delta\gamma},
\end{equation}

\noindent
where the Greek indices denote correlation types 
i.e. $\alpha,\beta,\delta,\gamma \in (g,+)$;
$z_{\rm s}$ identifies a particular redshift slices and $j,k$ are comoving scale bins.
The cross correlations between snapshots is potentially complicated, given that the
galaxy properties are strongly (but not fully) correlated.
However, since we do not attempt a fully simultaneous analysis across redshifts, but rather
restrict our inference to one snapshot at a time, we will neglect these additional
covariance terms.   
One can write each element as

\begin{multline}
\mathrm{Cov}\left[ w^{z_{\rm s}}_{\alpha \beta}(r_{\mathrm{p},i}), w^{z_{\rm s}}_{\delta \gamma}(r_{\mathrm{p},j}) \right ] =\\
\delta_{ij} \frac{2\pi}{\mathcal{A}_p r_{\mathrm{p},i} \Delta r_\mathrm{p} } 
\int k \mathrm{d}k 
\Theta_{\alpha \beta}(kr_{\mathrm{p},i}) \Theta_{\delta \gamma}(kr_{\mathrm{p},i}) \\
\left[ \tilde{P}_{\alpha \delta}(k, z_{\rm s})\tilde{P}_{\beta \gamma}(k, z_{\rm s})
+ \tilde{P}_{\alpha \gamma}(k, z_{\rm s})\tilde{P}_{\beta \delta}(k, z_{\rm s})
\right ],
\end{multline} 

\noindent
with the kernels

\begin{equation}
\Theta_{\mu\nu}(x) = 
\begin{cases}
J_2(x)          \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \mu\nu=g+ \\
J_0(x)          \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \mu\nu=gg \\
J_0(x) + J_4(x) \;\;\;\;\;                           \mu\nu=++ \\
\end{cases},
\end{equation}

\noindent
where $J_\nu$ is a Bessel function of the first kind of order $\nu$.
The covariance is, then, sensitive to both the IA signal and to cosmology
(via the power spectra $P(k)$).
In IA measurements on real data $\mathcal{A}_p$ is a function of
redshift, and accounts for the survey mask;
in our case it is simply the cross sectional area of the simulation
box in $h^{-2}$ Mpc$^{-2}$.
One should also note that the power spectra here are subject to a 
noise contribution, 

\begin{equation}
\tilde{P}_{\alpha \beta}(k, z_{\rm s}) = P_{\alpha \beta}(k, z_{\rm s}) + N^{z_{\rm s}}_{\alpha\beta},
\end{equation}

\noindent
where $N^{z_{\rm s}}_{\alpha \beta}=1/n^{z_{\rm s}}_{\rm c}$ for $\alpha \beta=gg$, 
$N_{\alpha \beta} = (\sigma^{z_{\rm s}}_e)^2/n^{z_{\rm s}}_{\rm c}$ for $\alpha \beta=++$,
and $N_{\alpha\beta}=0$ for $\alpha \beta=g+$.
The denominator $n_{\rm c}$ is the comoving volume number density of the
sample at $z=z_{\rm s}$ in $h^{3}$ Mpc$^{-3}$.

As is apparent from the above,
the analytic covariance matrix will depend to some 
extent on the input parameter values (cosmology, galaxy bias, and IAs).
As stated before, cosmological parameters are fixed to those 
appropriate for the simulation in question, as per Table \ref{tab:data:simulations}.
For the other (IA and bias) parameters,
we generate the fiducial matrix for each sample using an iterative
procedure similar to that of \citet*{y1methodology}.
That is, we repeatedly fit the data to obtain IA and galaxy bias
parameter constrains, update the covariance matrix and fit again.

Our convergence criteria are that (a) the marginalised 1D parameter 
posteriors are not systematically different between iterations, and 
(b) the $\chi^2$ and evidence values are stable to within a few
percent. 


We also test our fiducial analytic covariance matrix against a version
computed using jackknife resampling. It is worth bearing in mind that
the jackknife method is subject to a number of assumptions, not least
the statistical independence of subregions (see \citealt{anderson03,hartlap07} for discussion),
and that the scales of interest are much smaller than scale of the subregions.
These factors, combined with the relatively small number of subregions
allowed by even \tng~(the largest of the simulations considered here), are the
primary reason we consider jackknife as an approximate test of, and not
a viable alternative to, our analytic predictions. 
In the fiducial case (\tng), we divide the three dimensional box into
 $N_{\rm jk} = 4^3 = 64$ cubic subvolumes.
A visual comparison of the correlation matrices 
can be found in Figure \ref{fig:data:correlation_matrix}.
We also compare the root diagonals of the two covariance
matrices (see \ref{fig:app:covariance_comaprison}).
Although there is approximate agreement between the two, the jackknife method
tends to underestimate the variance on virtually all scales in the 
three correlations.
On the relevant scales for our fits ($>6\mpc$), the differences are
at the level of up to $\sim 50\%$ in $w_{g+}$.  




==> nla_theory.tex <==
The most common IA model is a hybrid prescription known as the Nonlinear Alignment (NLA) model;
in essence, the NLA model is an ad hoc alteration (see \citealt{bridle07}, \citealt{hirata07}) 
of an (at least partially, in certain regimes) 
physically motivated
prescription known as the Linear Alignment model \citep{catelan01, hirata04, hirata10}.
In this paradigm, one can write the intrinsic shape of a galaxy in terms of the 
background gravitational potential at the time of galaxy formation as:

\begin{equation}
(e^I_{+}, e^I_{\times}) = 
- \frac{C_1 }{4 \pi G} 
\left ( \frac{\partial^2 }{\partial x^2}-\frac{\partial^2 }{\partial y^2} ,
2 \frac{\partial^2}{\partial x \partial y} \right ) 
%\mathcal{S} \left [ 
\phi(\chi_{*}),
%\right ],
\end{equation}

\noindent
where $C_1$ is a normalisation constant, typically fixed at a
value of $5 \times 10^{-14} M_{\odot}^{-1} h^{-2}$ Mpc$^3$
\citep{brown02}. 
%The operator $\mathcal{S}$ represents a 
%filter, which smooths out density fluctuations on galactic 
%scales.
Following \citet{hirata04}, then, one can write the GI and II
power spectra in the form:

\begin{equation}\label{eq:theory:nla_gi}
P_{\rm GI} (k) \approx - \frac{C_1 \bar{\rho}(z)}{D(z)} a^2(z) P^{\rm lin}_\delta (k)
\end{equation}

\noindent
and 

\begin{equation}\label{eq:theory:nla_ii}
P_{\rm II} (k) \approx \left( \frac{C_1 \bar{\rho}(z)}{D(z)} \right )^2 a^4(z) P^{\rm lin}_\delta (k).
\end{equation}

\noindent
Here $\bar{\rho}$ is the (spatially averaged) mean matter density of the Universe
and $D$ is the linear growth function. The model also predicts higher order contributions,
as well as non-zero B modes arising from galaxy clustering, though these are
expected to be small.
We follow many previous analyses in fixing $C_1$ to \citet{brown02}'s value, 
but parameterising deviations in
strength of alignment from this baseline with a free amplitude, such that
$P_{\rm GI} \rightarrow A_1 P_{\rm GI}$
and
$P_{\rm II} \rightarrow A^2_1 P_{\rm II}$.

The innovation that defines the NLA is simply to replace the linear power spectrum
in Eq. \eqref{eq:theory:nla_gi} and \eqref{eq:theory:nla_ii} with the nonlinear
version. 
Though without physical justification,
%(indeed, being contradictory with the physical premise of the LA model),
this modification appears to improve the performance of the model on
small to intermediate scales (see, for example \citealt{bridle07, blazek15, singh15}).

Our fits using the NLA model incorporate all points in the range
$6 < \rp < L/3$ \mpc, where $L$ is the size of the simulation box in question.

==> results_tatt.tex <==
Interesting stuff about the TATT model fits.




\begin{figure}
\includegraphics[width=\columnwidth]{figures/tatt/c1_c2_redshift.pdf}
\includegraphics[width=\columnwidth]{figures/tatt/ai_redshift.pdf}
\caption{\emph{Upper}: TATT model parameter constraints from \fidsim~at four
redshifts. The minimum scale used in these fits was $\rp > 6 \mpc$.
\red{no B-modes}
}\label{fig:results:tatt:redshift_contours}
\end{figure}

==> tatt_theory.tex <==

We employ a second IA model, related to, but more complex than,
the NLA model. 
This prescription, referred to as the Tidal Alignment + 
Tidal Torque (TATT) Model was first proposed by \citet{blazek17}
and has been implemented a number of times in the context of 
cosmic shear analyses in the recent past 
(see \citealt{y1cosmicshear}).
We will provide a brief overview of the theory,
and refer the reader to those papers a more detailed
description.  

In this framework, a galaxy's intrinsic 
shape\footnote{The intrinsic shape here is defined
in an analogous way to the projected
ellipticity; it is the trace-free component of the
moment matrix in three dimensions, 
or equivalently, the eigenvector matrix of the 
3D inertia tensor. As noted in \citet{blazek17},
it is not a uniquely defined quantity, and depends 
on the radial weighting of the measurement algorithm.}
is written as an expansion in the trace-free 
tidal field tensor $s_{ij}$ :

\begin{equation}\label{eq:theory:expansion}
\gamma^I_{ij} = 
\underbrace{C_1 s_{ij} } _{\text{ Tidal Alignment }}
+ 
\underbrace{C_{1\delta} (\delta \times s_{ij} ) }_{\text{Density Weighting}}
+ 
\underbrace{C_2 \left [ \sum^2_{k=0} s_{ik} s_{kj} - \frac{1}{3} s^2 \right ]}_{\text{Tidal Torquing}}
 + \dots,
\end{equation}

\noindent
with both sides of the equation evaluated at a position $\mathbf{x}$,
which may be either a Lagrangian or an Eulerian position.
The two amplitudes $C_1$ and $C_2$ describe the magnitude
of alignment due to tidal alignment and tidal torquing respectively.
The term, with the coefficient $C_{1\delta}$, arises from
the fact that the observed alignment signal is effectively
weighted by the galaxy density, due to the fact that one can
only measure galaxy shapes in a position where there is actually
a galaxy. Note that the product of the matter overdensity and tidal
fields $\delta \times s_{ij}$ implicitly assumes a smoothing scale,
a detail we will return to in Section \ref{sec:daff}. 
It is worth bearing in mind, however, that these terms can absorb IAs
due to other mechanisms when fit to real data; 
for example, an effective non-zero $C_1$ can  
in principle arise in a pure tidal torquing IA scenario, 
when combined with nonlinear growth.

The real space dark matter 
tidal tensor is a $3\times3$ matrix 
defined as the trace free component of the
Hessian matrix of the smoothed
dark matter potential $\phi$ at $\mathbf{x}$. That is:

\begin{equation}
s_{ij}(\mathbf{x}) = \left ( \partial_i \partial_j - \delta_{ij} \frac{1}{3} \nabla^2 \right ) \phi ( \mathbf{x} ) ,
\end{equation}

\noindent
If the tidal tensor is computed using the nonlinear matter field,
then the former is equivalent to the NLA amplitude $A_{\rm IA}$.
Note that in order to constrain the different TATT amplitudes (Eq. \eqref{eq:theory:expansion}), 
we need to explicitly measure both the dark matter and the stellar tidal tensors
separately, rather than the overall matter (dark+stellar) version. 

Following \citet{blazek17}, our fits assume the density weighting term 
is related to the tidal alignment amplitude via a bias coefficient
(i.e. $C_{1\delta} = b_{\rm TA} C_1$).
Although in principle $b_{\rm TA}$ correspondes to the galaxy bias
of the source galaxies, given the interplay with the other 
parameters, it is more useful to think of it as an effective
IA parameter. 
As with the other terms,
$C_{1\delta}$ 
can be thought of more generally as describing any 
alignment physics with effective
large-scale correlations that depend on $s^g_{ij}$, 
and so does not necessarily correspond directly
to the galaxy bias constrained by $w_{gg}$,
as per the density weighting prediction.
Previous studies have chosen to fix it to one
(\citealt{y1cosmicshear}, \citealt{blazek17}),
and indeed \citet{y1coloursplit}, show that this decision is
not a significant source of uncertainty in the context of
$3\times2$pt cosmology.
This is not trivially true in our case, and we choose to
marginalise over this parameter in all our TATT fits.


One then has:

\begin{equation}
C_1 = - A_1 \bar{C}_1 \frac{\omegam \rho_{\rm crit}}{D(z)},
\end{equation}


\noindent
and

\begin{equation}
C_2 = 5 A_2 \bar{C}_1 \frac{\omegam \rho_{\rm crit}}{D^2(z)}.
\end{equation}


\noindent
The IA power spectra (GI and II) are derived from perturbation theory and are given
by integrals over the matter power spectrum; 
for details see Sections A-C of \citet{blazek17}.
Our version of the TATT model is identical to that of 
\citet{y1cosmicshear}, \citet{blazek17} and \citet{y1coloursplit}.
%(barring minor code updates in the intervening years).
It makes use of 
the \blockfont{FAST-PT} code \citep{mcewen16,fang17}, and is 
implemented within \blockfont{CosmoSIS}.

Finally, we note that the TATT model also predicts a non-zero B-mode term,
which enters the II power spectrum, and is sensitive to $C_{1 \delta}$ and $C_{2}$
(see \citealt{blazek17}, eq. 37-39).
These contributions are included in our modelling.
In Appendix C of that paper we demonstrate that this choice has negligible
impact on parameter constraints in the context of a DES Y1 $3\times2$pt
analysis. This is not trivially true for the type of measurement considered
in this work, and so we include all terms when fitting the TATT model here. 

The default minimum scale used in fits to the TATT model is $6h^{-1}$ Mpc,
but we explore the impact of this, and the potential viability of the 
model on smaller scales in Section \ref{sec:results:scales}. 

